CoRNStack: High-Quality Contrastive Data for Better Code Retrieval and Reranking

Effective code retrieval plays a crucial role in advancing code generation, bug fixing, and software maintenance, particularly as software systems increase in complexity. While current code embedding models have demonstrated promise in retrieving code snippets for small-scale, well-defined tasks, they often underperform in more demanding real-world applications such as bug localization within GitHub repositories. We hypothesize that a key issue is their reliance on noisy and inconsistent datasets for training, which impedes their ability to generalize to more complex retrieval scenarios. To address these limitations, we introduce CoRNStack, a large-scale, high-quality contrastive training dataset for code that spans multiple programming languages. This dataset is curated using consistency filtering to eliminate noisy positives and is further enriched with mined hard negatives, thereby facilitating more effective learning. We demonstrate that contrastive training of embedding models using CoRNStack leads to state-of-the-art performance across a variety of code retrieval tasks. Furthermore, the dataset can be leveraged for training code reranking models, a largely underexplored area compared to text reranking. Our finetuned code reranking model significantly improves the ranking quality over the retrieved results. Finally, by employing our code retriever and reranker together, we demonstrate significant improvements in function localization for GitHub issues, an important component of real-world software development.

==> figures/quality_prompt.tex <==
    % \begin{tcblisting}{
    %     listing only, 
    %     halign=left,
    %     listing engine=listings,
    %     title=\textbf{\small Prompt for SQL case study},
    %     colbacktitle=blue!30!white, 
    %     coltitle=black,
    %     left=0pt,               % Left inner padding
    %     right=0mm,              % Right inner padding
    %     top=0mm,                % Reduce top margin
    %     bottom=0mm,             % Reduce bottom margin
    %     boxsep=1mm,
    %     width=\textwidth,
    %     listing options={style=EBNF},
    %     label={fig:overview_grammar},
    % }
    % db_id: concert_singer
    % db_info: # stadium ( stadium_id , location , name , capacity , highest , lowest , average )
    % # singer ( singer_id , name , country , song_name , song_release_year , age , is_male )
    % # concert ( concert_id , concert_name , theme , stadium_id , year )
    % # singer_in_concert ( concert_id , singer_id )
    % # concert.stadium_id = stadium.stadium_id
    % # singer_in_concert.singer_id = singer.singer_id
    % # singer_in_concert.concert_id = concert.concert_id

    % question: How many singers do we have? Only output the SQL query. 
    % SQL:
    % \end{tcblisting}
    % \label{fig:database_schema_query}

==> tables/function_mrr.tex <==

% E5 19.76 5.91

% \begin{table*}[bt]
% \centering
% %\captionsetup{justification=centering}
% \label{table:main_function}
% %\resizebox{0.98\textwidth}{!}{

% \begin{tabular}{@{}c|c|c c c c c c c|c|c@{}}
% \toprule
%  & & \multicolumn{7}{c|}{\textbf{CSN}} & \textbf{CoSQA} & \textbf{AdvTest}\\

% \textbf{Model} & \textbf{Model Size} & Python & Java & JS & PhP & Go & Ruby & Avg. & Python & Python \\
% \midrule 
% UnixCoder & 125M & 42.17 & 43.92 & 40.46 & 35.21 & 61.39 & 55.22 & 42.11 & 27.32 \\
% OpenAI-Ada-002 & Unknown & 68.02 & 71.49 & 67.50 & 60.62 & 85.63 & 74.20 & 71.25 & 44.23 & 38.08 \\
% Amazon-CodeSage-Small & 130M & 64.38 & 63.19 & 60.01 & 54.71 & 77.66 & 63.20 & 64.86 & 49.92 & 41.28 \\
% CodeSage-Base & 356M & 67.99 & 68.02 & 66.95 & 58.15 & 83.21 & 68.00 & 68.72 & 48.50 & 49.08\\
% CodeSage-Large & 1.3B & 70.77 & 70.21 & 69.50 & 61.33 & 83.71 & 71.92 & 71.24 & 47.53 & 52.67\\
% Jina-Embeddings-v2-Base-Code & 161M & 64.40 & 66.40 & 61.76 & 55.94 & 84.4 & 70.4 & 67.22 & \textbf{67.78} & 37.06 \\
% Voyage-Code-2 & Unknown & 66.76 & 64.79 & 63.39 & 51.95 & 88.92 & 74.96 & 68.46 & 43.21 & - \\
% Salesforce-CodeT5+-Embedding & 110M & 71.72 & 71.83 & 69.17 & 67.82 & 90.73 & 74.45 & 74.23 & 40.09 & 40.82 \\
% Salesforce-CodeT5+-Matching & 220M & 74.17 & 74.76 & 70.17 & 68.6 & 91.37 & 76.04 & 75.85 & 51.51 & 42.9 \\
% \midrule 
% \textbf{Snowflake-Embed-Finetune} & 137M & \textbf{78.06} & \textbf{76.77} & \textbf{71.28} & \textbf{68.64} & \textbf{92.43} & \textbf{79.09} & \textbf{77.71} & 59.19 & \textbf{57.1} \\

% \end{tabular}
% \caption{Retrieval performance (MRR) on function-level code datasets}
% \label{tab:codesearchnet}

% \end{table*}

\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{}c|c|c c c c c c c|c@{}}
\toprule
 \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Retriever}}}& \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Param.}}}& \multicolumn{7}{c|}{\textbf{CodeSeachNet}} & \textbf{AdvTest}\\

 & & Python & Java & JS & PhP & Go & Ruby & Avg.  & Python \\
\midrule 
% UnixCoder & 125M & 42.2 & 43.9 & 40.5 & 35.2 & 61.4 & 55.2 & 42.1 & 27.3 \\
E5-Base & 110M & 11.2 & 9.0 & 8.9 & 8.6 & 25.6 & 16.8 & 13.4  & 5.9 \\
Arctic-Embed-M & 137M & 53.8 & 49.5 & 46.3 & 41.1 & 71.9 & 57.9 & 53.4 & 34.1 \\
% E5-Mistral & 7B & 11.2 & 9.0 & 8.9 & 8.6 & 25.6 & 16.8 & 13.4 & 4.0 \\
CodeSage-Small & 130M & 64.4 & 63.2 & 60.0 & 54.7 & 77.7 & 63.2 & 64.9 & 41.3 \\
CodeSage-Base & 356M & 68.0 & 68.0 & 67.0 & 58.2 & 83.2 & 68.0 & 68.7 & 49.1 \\
CodeSage-Large & 1.3B & 70.8 & 70.2 & 69.5 & 61.3 & 83.7 & 71.9 & 71.2 & 52.7 \\
Jina-Code-v2 & 161M & 64.4 & 66.4 & 61.8 & 55.9 & 84.4 & 70.4 & 67.2 & 37.1 \\
CodeT5+ & 110M & 71.7 & 71.8 & 69.2 & 67.8 & 90.7 & 74.4 & 74.2 & 40.8 \\
%CodeT5+-Matching & 220M & 74.2 & 74.8 & 70.2 & 68.6 & 91.4 & 76.0 & 75.9 & 51.5 & 42.9 \\
OpenAI-Ada-002 & Unknown & 68.0 & 71.5 & 67.5 & 60.6 & 85.6 & 74.2 & 71.3 & 38.1 \\
Voyage-Code-002 & Unknown & 66.8 & 64.8 & 63.4 & 52.0 & 88.9 & 75.0 & 68.5 & - \\
\midrule 
\textsc{CodeRankEmbed} & 137M & \textbf{78.4} & \textbf{76.9} & \textbf{71.4} & \textbf{68.8} & \textbf{92.7} & \textbf{79.3} & \textbf{77.9} & \textbf{59.5} \\
\bottomrule
\end{tabular}
\vspace{-0.5em}
\caption{Ranking performance (\%) for retrievers of difference sizes on function-level text-to-code retrieval datasets. Following~\cite{zhangcode}, we report numbers for MRR@1000.}
\label{tab:codesearchnet}
\end{table}

% \begin{table}[]
% \centering
% \footnotesize
% \label{table:main_function}
% \begin{tabular}{@{}c|c|c c c c c c c|c|c@{}}
% \toprule
%  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}}& \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Param.}}}& \multicolumn{7}{c|}{\textbf{CodeSeachNet}} & \textbf{CoSQA} & \textbf{AdvTest}\\

%  & & Python & Java & JS & PhP & Go & Ruby & Avg. & Python & Python \\
% \midrule 
% % UnixCoder & 125M & 42.2 & 43.9 & 40.5 & 35.2 & 61.4 & 55.2 & 42.1 & 27.3 \\
% E5-Base & 110M & 11.2 & 9.0 & 8.9 & 8.6 & 25.6 & 16.8 & 13.4 & 19.8 & 5.9 \\
% Arctic-Embed-M & 137M & 53.8 & 49.5 & 46.3 & 41.1 & 71.9 & 57.9 & 53.4 & 56.3 & 34.1 \\
% E5-Mistral & 7B & 11.2 & 9.0 & 8.9 & 8.6 & 25.6 & 16.8 & 13.4 & 12.6 & 4.0 \\
% CodeSage-Small & 130M & 64.4 & 63.2 & 60.0 & 54.7 & 77.7 & 63.2 & 64.9 & 49.9 & 41.3 \\
% CodeSage-Base & 356M & 68.0 & 68.0 & 67.0 & 58.2 & 83.2 & 68.0 & 68.7 & 48.5 & 49.1 \\
% CodeSage-Large & 1.3B & 70.8 & 70.2 & 69.5 & 61.3 & 83.7 & 71.9 & 71.2 & 47.5 & 52.7 \\
% Jina-Code-v2 & 161M & 64.4 & 66.4 & 61.8 & 55.9 & 84.4 & 70.4 & 67.2 & \textbf{67.8} & 37.1 \\
% CodeT5+ & 110M & 71.7 & 71.8 & 69.2 & 67.8 & 90.7 & 74.4 & 74.2 & 40.1 & 40.8 \\
% %CodeT5+-Matching & 220M & 74.2 & 74.8 & 70.2 & 68.6 & 91.4 & 76.0 & 75.9 & 51.5 & 42.9 \\
% OpenAI-Ada-002 & - & 68.0 & 71.5 & 67.5 & 60.6 & 85.6 & 74.2 & 71.3 & 44.2 & 38.1 \\
% Voyage-Code-2 & - & 66.8 & 64.8 & 63.4 & 52.0 & 88.9 & 75.0 & 68.5 & 43.2 & - \\
% \midrule 
% \textbf{Ours} & 137M & \textbf{78.4} & \textbf{76.9} & \textbf{71.4} & \textbf{68.8} & \textbf{92.7} & \textbf{79.3} & \textbf{77.9} & 58.3 & \textbf{59.5} \\
% \bottomrule
% \end{tabular}
% \caption{Retrieval performance (MRR@1000 in \%) on function-level text-to-code retrieval datasets.}
% \label{tab:codesearchnet}

